On a class of three-dimensional integrable Lagrangians

We characterize non-degenerate Lagrangians of the form $ \int f(u_x, u_y, u_t) dx dy dt $ such that the corresponding Euler-Lagrange equations $ (f_{u_x})_x+ (f_{u_y})_y+ (f_{u_t})_t=0 $ are integrable by the method of hydrodynamic reductions. The integrability conditions constitute an over-determined system of fourth order PDEs for the Lagrangian density $f$, which is in involution and possess interesting differential-geometric properties. The moduli space of integrable Lagrangians, factorized by the action of a natural equivalence group, is three-dimensional. Familiar examples include the dispersionless Kadomtsev-Petviashvili (dKP) and the Boyer-Finley Lagrangians, $f=u_x^3/3+u_y^2-u_xu_t$ and $f=u_x^2+u_y^2-2e^{u_t}$, respectively. A complete description of integrable cubic and quartic Lagrangians is obtained. Up to the equivalence transformations, the list of integrable cubic Lagrangians reduces to three examples, $ f=u_xu_yu_t, f=u_x^2u_y+u_yu_t, and f=u_x^3/3+u_y^2-u_xu_t ({\rm dKP}).$ There exists a unique integrable quartic Lagrangian, $ f=u_x^4+2u_x^2u_t-u_xu_y-u_t^2.$ We conjecture that these examples exhaust the list of integrable polynomial Lagrangians which are essentially three-dimensional (it was verified that there exist no polynomial integrable Lagrangians of degree five). We prove that the Euler-Lagrange equations are integrable by the method of hydrodynamic reductions if and only if they possess a scalar pseudopotential playing the role of a dispersionless `Lax pair'. MSC: 35Q58, 37K05, 37K10, 37K25. Keywords: Multi-dimensional Dispersionless Integrable Systems, Hydrodynamic Reductions, Pseudopotentials.

==> 1-README <==
In this file we describe the contents of the attached files.

The LaTeX file of the paper is "FKT-3dimL.tex".

00README.XXX is a file needed for the automated
 arxive.org processing system - ignore it!

The file "progs.tar" contains the program files
necessary to perform the computations used
in Sections 2 and 4 of the paper.

Most of the computations were performed by using a free
symbolic computation systems FORM, version 3.1. Its complete 
distribution as well as tutorials and the reference
manual are downloadable from 
http://www.nikhef.nl/~form/

Some computations in this paper were performed by using Maple(TM).
Maple is a trademark of Waterloo Maple Inc.

The actual programs were run on Macintosh PowerPC G4 
(1.3 GHz, 512 Mb RAM)
and required from 1 to 15 minutes CPU time each.

All program files are tar-compressed so please do
tar -xvf progs.tar
to uncompress them.
The files with Maple code (Maple text input) have the extension "mpl".
The files with FORM code have the extension "frm".
We have included the log-files of FORM runs for the main
parts of the computations, they are gzip-compressed and have
the extension *.log.gz

The contents of the files:

1-README - this file

2-Lagr3dim.frm  - the main file for derivation of
                the equations for the Lagrangian,
                it performs the most of the computations
                necessary to prove Theorem 1 (Section 2).
                It contains explanation of the used notations
                and comments the main steps of the simplification
                procedures. The result of this computation
                is stored in internal FORM format in the file "all.sav"
                and in Maple text input format in "3-Lagr3dim4maple".

4-solveEq.mpl - this Maple program solves the system of 45
                equations for the 15 derivatives of the Lagrangian
                of order 4. The result is stored in Maple text input
                format in the file "f4ord.mpl" and in FORM text input
                format in the file "f4ord.frm".
                We check that these data give the correct
                solution of the system obtained in "2-Lagr3dim.frm"
                by a substitution in the file "f4ord-test-sol.frm".

f4ord-test-compat.frm - we test here that the expressions for
                       the fourth order derivatives of the Lagrangian
                       give an involutive system (are compatible).

7-final-form.mpl - here we check that the expressions for
                  the fourth order derivatives of the Lagrangian
                  are equivalent to the form (2) given
                  in the paper.

The files performing the computations necessary to prove
Theorem 2 (Section 4) are collected below. The straighforward
Maple computation of the second-order derivatives of F(a,b,c,\xi)
(in terms of its first-order derivatives and the derivatives
of the Lagrangian) is not included, as well as the huge results
of this computation: they occupy more than 5 megabytes
in FORM text input format and are in fact not necessary:
we give the simplified expressions (in the file "F2ordReduced",
FORM text input format) and check in "5-test-F2-reduced.frm"
that they ARE the needed expressions modulo the relation (23).
The simplification procedure is given in 
"psevdopot-F2ord-simplification.frm" just for reference.
In the FORM program "6-pseudopot-F3.frm"
we form the 3rd-order compatibility conditions for F
and check that they are satisfied modulo the 4th-order 
relations (2) for the Lagrangian. The fact that these compatibility
conditions are equivalent to (2) was checked by a straighforward
Maple program; it simply verified that the matrix 
of the coefficients of 4th-order derivatives of the Lagrangian
in these compatibility conditions have the necessary rank 15.


